PaMO: Parallel Mesh Optimization for Intersection-Free Low-Poly Modeling on the GPU

Reducing the triangle count in complex 3D models is a basic geometry preprocessing step in graphics pipelines such as efficient rendering and interactive editing. However, most existing mesh simplification methods exhibit a few issues. Firstly, they often lead to self-intersections during decimation, a major issue for applications such as 3D printing and soft-body simulation. Second, to perform simplification on a mesh in the wild, one would first need to perform re-meshing, which often suffers from surface shifts and losses of sharp features. Finally, existing re-meshing and simplification methods can take minutes when processing large-scale meshes, limiting their applications in practice. To address the challenges, we introduce a novel GPU-based mesh optimization approach containing three key components: (1) a parallel re-meshing algorithm to turn meshes in the wild into watertight, manifold, and intersection-free ones, and reduce the prevalence of poorly shaped triangles; (2) a robust parallel simplification algorithm with intersection-free guarantees; (3) an optimization-based safe projection algorithm to realign the simplified mesh with the input, eliminating the surface shift introduced by re-meshing and recovering the original sharp features. The algorithm demonstrates remarkable efficiency, simplifying a 2-million-face mesh to 20k triangles in 3 seconds on RTX4090. We evaluated the approach on the Thingi10K dataset and showcased its exceptional performance in geometry preservation and speed.

==> sec/figure_only.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{figs/baseline_inter.pdf}
\caption{\textbf{Qualitative Comparison with Baseline Methods.} We visualize both the front and back of an object. Our method guarantees intersection-free output meshes, whereas baseline models cannot avoid producing self-intersecting triangles (denoted in red). }
\label{fig:baseline_inter}
\end{figure*}

% How our Edge cost affects to aviod skinny triangle
% TODO : Add Quantitative result
% Original : the local region before collapsing
% figure to compare threshold 0.0001, 0.001, 0.01, 0.1, 1
% TODO : test on more thresholds, maybe multiple pair of curves, each pair is a threshold
\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{figs/threshold_comp_new.pdf}

  \caption{\textbf{Different Level of Details.} We examined the results of Chamfer Distance (CD) and Hausdorff Distance (HD) by applying different levels of detail to the same mesh. It was observed that when the mesh is simplified beyond 1\% of the original number of faces, there is a sharp increase in CD and HD. This is due to the fact that in smaller meshes, multiple edges can cause self-intersections or induce invalid collapses. In order to further simplify the mesh to the target ratio, a list of invalid edges continues to accumulate. Consequently, edges with relatively higher costs are selected for collapsing.}
  \label{fig:threshold_comp}
\end{figure*}

\begin{figure*}[tb]
\begin{center}
   \includegraphics[width=\linewidth]{figs/sharp_feat_v2.pdf}
\end{center}
  \caption{\textbf{Effectiveness of safe projection. }Safe projection recovers sharp corners and edges from our simplified mesh, matching input geometry more closely.}
  \label{fig:sharp_feat}
\end{figure*}

\begin{figure}[t]
\centering
\includegraphics[width=1.0\linewidth]{figs/undo_remesh_new.png}
  \caption{Impact of Remeshing on Simplification Performance. \textbf{Left:}
  number of edge collapses reversed by undo operation each iteration. \textbf{Right:} Number of edges remaining after each parallel edge collapse iteration.
  We conduct tests on a mesh with 450k faces, which includes many skinny triangles, to observe the differences in the simplification process with and without remeshing. Even though the number of edges increases from 100k to 700k after remeshing, there is a significant difference in the rate of mesh reduction. We observe that without remeshing, numerous edges require undo operation each iteration, and with remeshing, undo is not needed at all during the experiment, leading to faster edge count reduction.}
  
\label{fig:undo_remesh}
\end{figure}



\newpage



\begin{figure}[t]
\begin{center}
   \includegraphics[width=1.0\linewidth]{figs/runtime_distribution.png}
\end{center}
  \caption{Runtime distribution of our pipeline over the entire Thingi10K dataset. Note that we exclude 5 corrupted input meshes in the dataset.}
\label{fig:runtime_10k}
\end{figure}

\begin{figure}[t]
\begin{center}
   \includegraphics[width=1.0\linewidth]{figs/edge_cost.pdf}
\end{center}
  \caption{Ablation study on the extra metrics in the edge computation. Both edge length and skinny cost metrics can effectively reduce the appearance of skinny triangles. We assess their improvement by calculating the minimum angle of triangles within the output mesh.}
\label{fig:edge_cost}
\end{figure}

==> tables/Analysis_ours.tex <==
\begin{table*}[htbp]
\small
\centering
\caption{Analysis of our algorithm}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\toprule
\# of faces & \multicolumn{2}{c|}{Time / ms} & \multicolumn{2}{c|}{\# of converge} & \multicolumn{2}{c|}{\# faces after converge} & \multicolumn{2}{c|}{avg \# of undo edges} & \multicolumn{2}{c|}{avg \# of undo iteration} & \multicolumn{2}{c|}{worst \# undo operation} & \multicolumn{2}{c}{rate of intersect} \\
\cmidrule(l){2-3} \cmidrule(l){4-5} \cmidrule(l){6-7} \cmidrule(l){8-9} \cmidrule(l){10-11} \cmidrule(l){12-13} \cmidrule(l){14-15}
 & avg & std & avg & std & avg & std & avg & std & avg & std & avg & std & avg & std \\
\midrule
2M & & & & & & & & & & & & & & \\
1.5M & & & & & & & & & & & & & & \\
700k & & & & & & & & & & & & & & \\
200k & & & & & & & & & & & & & & \\
\bottomrule
\end{tabular}
\label{tab:runtime_comp}
\end{table*}


==> tables/projection_chamfer.tex <==
\begin{table}[htbp]
\small
  \centering
  \caption{Chamfer distance between the results with GT mesh from different stages.}
    \begin{tabular}{l|ccc}
    \toprule
        Stage & Chamfer Distance \\
    \midrule
    Stage 1 &  \\
    Stage 2 & \\
    Stage 3 & \\
    \bottomrule
    \end{tabular}
  \label{tab:proj_cd}
\end{table}

